Deterministic Vertex Connectivity via Common-Neighborhood Clustering and Pseudorandomness

We give a deterministic algorithm for computing a global minimum vertex cut in a vertex-weighted graph $n$ vertices and $m$ edges in $\widehat O(mn)$ time. This breaks the long-standing $\widehat \Omega(n^{4})$-time barrier in dense graphs, achievable by trivially computing all-pairs maximum flows. Up to subpolynomial factors, we match the fastest randomized $\tilde O(mn)$-time algorithm by [Henzinger, Rao, and Gabow'00], and affirmatively answer the question by [Gabow'06] whether deterministic $O(mn)$-time algorithms exist even for unweighted graphs. Our algorithm works in directed graphs, too. In unweighted undirected graphs, we present a faster deterministic $\widehat O(m\kappa)$-time algorithm where $\kappa\le n$ is the size of the global minimum vertex cut. For a moderate value of $\kappa$, this strictly improves upon all previous deterministic algorithms in unweighted graphs with running time $\widehat O(m(n+\kappa^{2}))$ [Even'75], $\widehat O(m(n+\kappa\sqrt{n}))$ [Gabow'06], and $\widehat O(m2^{O(\kappa^{2})})$ [Saranurak and Yingchareonthawornchai'22]. Recently, a linear-time algorithm has been shown by [Korhonen'24] for very small $\kappa$. Our approach applies the common-neighborhood clustering, recently introduced by [Blikstad, Jiang, Mukhopadhyay, Yingchareonthawornchai'25], in novel ways, e.g., on top of weighted graphs and on top of vertex-expander decomposition. We also exploit pseudorandom objects often used in computational complexity communities, including crossing families based on dispersers from [Wigderson and Zuckerman'99; TaShma, Umans and Zuckerman'01] and selectors based on linear lossless condensers [Guruswwami, Umans and Vadhan'09; Cheraghchi'11]. To our knowledge, this is the first application of selectors in graph algorithms.

==> balanced-case.tex <==

\section{Algorithms for Balanced Cases: Applications of Pseudorandom Objects} \label{sec:application of pseudorandom objects}

In this section, we will apply the theorems for pseudorandom objects (i.e.,~\cref{thm:crossing family,thm:selector}) to efficiently solve vertex connectivity when the minimum cut $(L,S,R)$ has some idealistic balanceness guarantees. The lemmas proved in this section will serve as important subroutines in the following subsections.

We first need to introduce the vertex version of the isolating cuts lemma, which is from \cite{li_vertex_2021}.

\begin{lemma}[Lemma 4.2 of \cite{li_vertex_2021}]\label{isolatingvertexcuts}
There exists an algorithm that takes an input graph $G=(V, E)$ and an independent set $I \subset V$ of size at least 2, and outputs for each $v \in I$, a $({v}, I\setminus {v})$-min-separator $C_v$.
The algorithm makes $(s,t)$ max-flow calls on unit-vertex-capacity graphs with $O(m\log |I|)$ total number of vertices and edges and takes $O(m)$ additional time.
\end{lemma}


The following lemma is an application of selector~\cref{thm:selector} and  crossing family~\cref{thm:crossing family},  which shows $\kappa$ calls to max flow are possible when $|L|$ is roughly the same as $|S|$ and $|R|$ larger than $|S|$.

\begin{lemma}\label{lem:balancedterminalalgorithm}
    There is a deterministic algorithm \textsc{BalancedTerminalVC}$(G,T,k)$ that takes as inputs an undirected graph $G=(V,E)$, a terminal set $T\subseteq V$ and a cut parameter $k$, outputs a vertex cut of $G$. If there exists a vertex cut $(L,S,R)$ of $G$ such that $|T\cap L|,|T\cap R|=\widehat{\Omega}(|T\cap S|)$ and $|T\cap L|=\widehat{O}(k)$, then the output cut is a minimum vertex cut of $G$. The algorithm runs in $\widehat{O}(mk)$ time.
\end{lemma}
\begin{proof}


    Suppose $|T\cap L|\le k\cdot n^{g(n)}$ and $|T\cap L|,|T\cap R|\ge n^{-g(n)}\cdot |T\cap S|$ where $g(n)=o(1)$. Let $\eps=n^{-2g(n)}$ and let $\cS$ be a $(|T|,k/\epsilon,\epsilon)$-selector which is a family of subsets of $[|T|]$. Here we map each number in $1,...,|T|$ to a vertex in $T$, and with a little abuse of notation, each $X\subseteq\cS$ is a vertex subset of $T$. Let $\alpha=\max(1/\sqrt{\log n},\sqrt{g(n)})$. Here we assume $k/\epsilon\le (|T|\epsilon/\log^2n)^{1/(1+\alpha)}$, the case when $k$ is large will be solved in the next paragraph. According to~\cref{thm:selector}, we can construct $\cS$ of size $|\cS|=k^{1+o(1)}\cdot n^{o(1)}$ in $\hO{n}$ time, and every set $X\subseteq\cS$ has size at least $|T|/|\cS|$. Here we require $n/|\cS|\ge 2$, we will show what to do when $|T|/|\cS|<2$ later. Notice that $k<|T\cap L|\le k/\epsilon$ and $|T\cap S|\le k/\epsilon$. Now according to the definition of selector, there exists $X\subseteq \cS$ such that $|X\cap L|=1$ and $|X\cap S|=0$ and $|X|\ge 2$. According to~\cref{isolatingvertexcuts}, by setting the independent set $I$ to be a maximal independent set of $X$, which must satisfy $|I\cap L|=1,|I\cap S|=0$ and $|I|\ge 2$, we can get a vertex cut of size at most $S$ since $S$ itself is an isolating cut. Notice that the running time is $\widehat{O}(m|\cS|)=\widehat{O}(mk)$.

    Now suppose $|T|/|\cS|<2$ or $k/\epsilon> (|T|\epsilon/\log^2n)^{1/(1+\alpha)}$, which means $k\cdot n^{o(1)}\ge |T|$. We construct an $(|T|,1/\epsilon,1/\epsilon)$-crossing family $\cP$ according to~\cref{thm:crossing family}. Similarly, we abuse the notation a bit and assume each $P\subseteq\cP$ is a subset of $T\times T$. According to the definition of crossing family, there exists $(s,t)\in P$ such that $s\in L,t\in R$. Thus, by running $s-t$ min cut over all $(s,t)\in P$ and find the minimum one, we get the minimum vertex cut of $G$. The algorithm runs in time $\hO{m|T|}$ which is fine since $k\cdot n^{o(1)}\ge |T|$.
\end{proof}

The following lemma is a more fine-grained version of~\cref{lem:balancedterminalalgorithm}, which works on a subgraph.

\begin{lemma}\label{lem:subgraphbalancedterminalalgorithm}
    There is a deterministic algorithm \textsc{SubgraphBalancedTerminalVC}$(G,T,k)$ that takes as inputs an undirected graph $G=(V,E)$, a terminal set $T\subseteq V$ and a cut parameter $k$, outputs a vertex cut of $G$. If there exists a vertex cut $(L,S,R)$ of $G$ such that $L\subseteq T$ and $|L|,|T\cap R|=\hat{\Omega}(|T\cap S|)$ and $|L|=\hat{O}(k)$ and $L\subseteq T$, then the output cut is a minimum vertex cut of $G$. The algorithm runs in $\hat{O}((k\sum_{t\in T}|N_{G}(t)|)$ time.
\end{lemma}

\begin{proof}
    The proof is similar to the proof of~\cref{lem:balancedterminalalgorithm}. Suppose $|T\cap L|=|L|\le k\cdot n^{g(n)}$ and $|L|,|T\cap R|\ge n^{-g(n)}\cdot |T\cap S|$ where $g(n)=o(1)$ and define $\epsilon$ and $\cS$ and $I$ in the same way as in the proof of~\cref{lem:balancedterminalalgorithm}. We will explain what to do when $|T|/|\cS|<2$ or $k$ is large later. Notice that $I$ has the property $|I\cap L|=1,|I\cap S|=0$ and $|I|\ge 2$. Now we cannot afford to run isolating cuts on the whole graph because we want the running time to be smaller. Instead, we construct a graph
    \[G'=(T\cup N_G(T)\cup \{s\},E(T,T\cup N_G(T))\cup \{(s,u)\mid u\in N_G(T)\}\]

    Define $I'=I\cup\{s\}$. The algorithm use~\cref{isolatingvertexcuts} on $I',G'$. The running time is bounded by $\widehat{O}((k\sum_{t\in T}|N_{G}(t)|)$ where $O(\sum_{t\in T}|N_{G}(t)|)$ is the size of $G'$. Now we prove that the minimum isolating cut of $I'$ (denoted by $C_v$ which is a $(v,I'\backslash v)$-min-separator for some $v\in I'$) on $G'$ is equal to $|S|$. Notice that $S=N_G(L)=N_{G'}(L)$ since $L\subseteq T$. Also, notice that $S\cap I'=\emptyset$. Thus, $S'$ is an isolating cut of $I'$, which means $|S|\ge |C_v|$. On the other way, suppose the connected component containing $v$ after deleting $C_v$ is $L_v$. We have $L_v\subseteq T$, otherwise $s\in N(L_v)$. Thus, we have $N_G(L_v)=N_{G'}(L_v)$. Notice that $N_G(L_v)\cup L_v\not=V$ since $|I|\ge 2$, and there must exists a vertex in $I$ other than $v$ inside $T$ outside $N_G(L_v)\cup L_v$. Thus, $C_v$ is a vertex cut of $G$, which implies $|S|\le |C_v|$.

    Now suppose $|T|/|\cS|<2$ or $k/\epsilon>(|T|\epsilon/\log^2n)^{1/(1+\alpha)}$, which means $k\cdot n^{o(1)}\ge |T|$. Similar to the proof of~\cref{lem:balancedterminalalgorithm}, we construct an $(|T|,1/\epsilon,1/\epsilon)$-crossing family $\cP$. There exists $(a,b)\in P$ such that $a\in L,b\in R$. Instead of running $(a,b)$ min cut on $G'$ over all $(a,b)\in P$, we run $(a,b\cup\{s\})$ min cut on $G'$. Any $(a,b\cup\{s\})$ min cut $(L',S',R')$ satisfying $L'\subseteq T$ since $s$ connects to all nodes in $N_G(T)$. Thus, $N_G(L')=N_{G'}(L')$ and $t\in R'$ where $t\in V$. Thus, $S'$ is a vertex cut of $G$. On the other hand, the minimum vertex cut $S$ of $G$ is also a vertex cut of $(a,b\cup\{s\})$ for some $(a,b)\in P$ since $L\subseteq T$. The total running time is $\widehat{O}(k\sum_{t\in T}|N_{G}(t)|)$.
\end{proof}


==> expanderSizing.tex <==
\section{Omitted Proofs from \texorpdfstring{\Cref{sec:pseudo random objects}}{Pseudorandom Objects}}

\begin{proof}[Proof of \Cref{clm:bigVertexExpander}]
    Let $X$ be the Ramanujan graph constructed with inputs $n$ and $d=\frac{64}{\eta}$. According to the guarantees of \Cref{lem:explicit ramanujan}, we know that $|V_X|\leq \cGabow n$ and it is $d'$-regular with $d \leq d' \leq 4d$. From \Cref{lem:RamanujanEigen}, we can conclude that the second eigenvalue of $X$, $\lambda_2(X) \leq 2\sqrt{d'-1}/d' \leq 2/\sqrt{d}$.

    Therefore, by setting $\alpha = \eta/16$ in \Cref{lem:spectralExpansion}, we can deduce that $X$ is a $(\eta/16, \beta)$ where $\beta = \frac{1}{(1-\eta/16)\lambda_2(X)^2 + \eta/16}-1 \geq \frac{1}{\frac{4}{d}+\eta/16}-1 \geq \frac{8}{\eta}-1 > 4/\eta$, given that $\cGabow\geq 1$ and $\eta < 1$. The construction time for the graph $X$ is at most $O(nd) = O(n/\eta)$.
\end{proof}

\begin{proof}[Proof of \Cref{clm:expanderSizing}]
    If $\rho$ is an integer, we obtain $H$ by contracting arbitrary groups of $\rho$ vertices in $G$. However, if $\rho$ is not an integer, we contract arbitrary groups of $\floor{\rho}$ or $\ceil{\rho}$ many vertices together to achieve a graph of size exactly $n$.

    Let $L_H\subset V_H$ is of size at most $\alpha n/\ceil{\rho}$. For each $v\in V_H$, let $C_v \subset V_G$ denote the vertices in $G$ contracted to form $v$. Uncontracting the set of vertices in $L_H$, we get $L_G = \cup_{v\in L_H} C_v$. We have $|L_G| \leq \ceil{\rho}|L_H| \leq \alpha n$, hence we have $|N_G(L_G)| \geq \beta |L_G|$ as $G$ is a $(\alpha,\beta)$-vertex expander.

    Let $C[N_G(L_G)] = \{v \in V_H \mid C_v \cap N_G(L_G) \neq \emptyset\}$ be the set of contracted vertices in $V_H$ such that corresponding set $C_v\subset V_G$ has at least one vertex from $N_G(L_G)$. Observe that $C[N_G(L_G)] = N_H(L_H)$. Every vertex in $C[N_G(L_G)]$ has at least one edge from a vertex in $L_H$ as the edge across $L_G$ and $N_G(L_G)$ is preserved after contraction. Hence, $C[N_G(L_G)]\subseteq N_H(L_H)$. Every vertex $v \in N_H(L_H)$ has a vertex $u \in L_H$ such that $(u,v)\in E_H$. Uncontracting $u,v$ we have every vertex $w\in C_v$ that has edges from some vertex $x\in C_u\subset L_G$ should belong to $N_G(L_G)$, hence $v\in C[N_G(L_G)]$ and we have $N_H(L_H)\subseteq C[N_G(L_G)]$.

    We have \[|N_H(L_H)| = |C[N_G(L_G)]|\geq \frac{|N_G(L_G)|}{\ceil{\rho}} \geq \frac{\beta |L_G|}{\ceil{\rho}} \geq \frac{\beta\floor{\rho}}{\ceil{\rho}}|L|.\] The first and third inequalities follow as we contract at most $\ceil{\rho}$ and at least $\floor{\rho}$ many vertices in $G$ to construct $H$. Hence, expansion is at least $\frac{\beta\floor{\rho}}{\ceil{\rho}}$.

    The time taken to contract arbitrary vertices is at most $O(m)$ by going over each edge and mapping them to the new contracted vertices.
\end{proof}


==> terminalreduction.tex <==
\section{Terminal Reduction Main Algorithm (\texorpdfstring{$\hat{O}(mk)$}{O(mk)} for Undirected Graph)} \label{sec:terminal main}

\newcommand{\balanced}[1]{#1-balanced}
\newcommand{\strongbalanced}[1]{#1-strongly-balanced}

We first define balanced terminal sets.
\begin{definition}\label{def:balancedterminalset}
    For an undirected graph $G=(V,E)$, a terminal set $T\subseteq V$ is called \emph{\strongbalanced{$\alpha$}} if for any minimum vertex cut of $G$ denoted by $S$ and any connected component of $G[V-S]$ denoted by $L$, we have $|T\cap L|\ge \alpha|S|$.
\end{definition}

In this section, we will prove the following lemma.

\begin{lemma}\label{lem:terminalreduction}
    There is a deterministic algorithm \textsc{TerminalReduction}$(G,T,k)$ (\cref{alg:terminalreduction}) that takes as inputs an $n$-vertex $m$-edge undirected graph $G=(V,E)$, along with a \strongbalanced{$2^{\sqrt{\log n}/2}$} terminal set $T\subseteq V$ and a cut parameter $k\ge\kappa_G$ and $k=O(\kappa_G)$, outputs $(S',T')$ where
    \begin{itemize}
        \item $|T'|\le 0.9|T|$,
        \item either $S'$ is a minimum vertex cut of $G$ or $T'\subseteq V$ is a \strongbalanced{$0.01$} terminal set.
    \end{itemize}
    The algorithm runs in time $\hat{O}(mk)$.
\end{lemma}
\begin{remark}
    In the overview part, we use the definition of ``$\alpha$-balanced'' (which only focuses on one minimum vertex cut $(L,S,R)$) instead of $\alpha$-strongly-balanced here because it makes the algorithm easier to explain. Another reason for the inconsistency is that our algorithm can keep every minimum vertex cut to be balanced, which is a stronger result that can have independent interests.
\end{remark}
With~\cref{lem:unbalanced,lem:terminalreduction}, we are ready to prove our main theorem for undirected graph.
\begin{proof}[Proof of~\cref{thm:main k max flows}]
    By~\cite{NagamochiI92}, we can assume the input undirected graph $G$ has number of edges $m=(\kappa_G n)$ by $O(m)$ time preprocessing. The minimum degree $\delta=O(\kappa_G)$ since the average degree is $O(\kappa_G)$. Notice that $\delta\ge\kappa_G$. Thus, by setting $k=\delta$ we have $k\ge\kappa_G$ and $k=O(\kappa_G)$.

    The algorithm first use \cref{lem:unbalanced} on $G$ to get a vertex cut $S^*$. Then the algorithm set $T_0=V$, and for $i=0,1,2,...$ run
    \[S_i\leftarrow\textsc{BalancedTerminalVC}(G,T_i,k)\] and
    \[(S'_i,T_{i+1})\leftarrow\textsc{TerminalReduction}(G,T_i,k)\] until $T_{i+1}$ becomes empty. The returned cut will be the minimum one among $S^*$ and $S_i,S'_i$ for all $i$.

    \paragraph{Correctness.} If there exists a minimum vertex cut $S$ and a minimum size connected component $L$ of $G[V-S]$ (that makes $|V-L-S|\ge |L|$) such that $|L|=O(|S|)=O(\delta)$, then according to~\cref{lem:unbalanced}, $S^*$ is a minimum vertex cut. Otherwise, let $i$ be the minimum index such that $T_i$ is not a \strongbalanced{$2^{\sqrt{\log n}/2}$} terminal set. If $i=0$, notice that $T_0=V$ which is a \strongbalanced{0.01} terminal set. If $i>0$, since $T_{i-1}$ is a \strongbalanced{$2^{\sqrt{\log n}/2}$} terminal set, according to~\cref{lem:terminalreduction}, either $S_{i-1}$ is a minimum vertex cut, or $T_i$ is a \strongbalanced{0.01} terminal set. In any case, $T_i$ is a \strongbalanced{0.01} terminal set and not a \strongbalanced{$2^{\sqrt{\log n}/2}$} terminal set, unless one of $S^*,S'_0,S'_1,...$ is a minimum vertex cut. By the definition, there exists a vertex cut $S$ and a connected component of $G[V-S]$ denoted by $L$ such that $|T_i\cap L|<2^{\sqrt{\log n}/2}|S|$. We also have $|T_i\cap L|>0.01|S|$ and $|V-S-L|>0.01|S|$. According to~\cref{lem:balancedterminalalgorithm}, $S_i$ is a minimum vertex cut of $G$.

    \paragraph{Complexity.} According to~\cref{lem:terminalreduction}, $|T_{i+1}|\le 0.9|T_i|$, so there can be at most $O(\log n)$ loop of algorithm. Each loop takes time $\hat{O}(m\kappa_G)$ according to~\cref{lem:terminalreduction,lem:balancedterminalalgorithm}.
\end{proof}

We need the following two lemmas as subroutines of our algorithm~\cref{alg:terminalreduction}.


\begin{lemma}[Vertex expander decomposition, \cite{LongS22}]\label{lem:vertexexpanderdecomposition}
    There is a deterministic algorithm \textsc{ExpanderDecomposition}$(G,T)$ that takes as inputs an $n$-vertex $m$-edge undirected graph $G=(V,E)$ and a terminal set $T\subseteq V$, return $(X,\mathcal{U})$ where $X\subseteq V$ and $\mathcal{U}$ is a set of subsets of $V$, such that
    \begin{enumerate}
        \item $X$ along with all sets in $\mathcal{U}$ form a partition of $V$, i.e., they are disjoint and the union of them is $V$,
        \item there are no edges between different sets in $\mathcal{U}$, i.e., $E(U_1,U_2)=\emptyset$ for any $U_1,U_2\in \mathcal{U}$ with $U_1\not=U_2$,
        \item $G[U]$ is a $(T,2^{-\log^{0.1} n})$-vertex expander for any $U\in\mathcal{U}$,
        \item $|X|<0.01|T|$.
    \end{enumerate}
    The algorithm runs in time $\hat{O}(m)$.
\end{lemma}

\begin{lemma}\label{lem:shaving}
    There is a deterministic algorithm \textsc{Shaving}$(G,A,a)$ that takes as inputs an undirected graph $G=(V,E)$, a vertex set $A$ and a integer $a$, return $R\subseteq A$ such that
    \begin{itemize}
        \item if there exists $B\subseteq V$ and $A'\subseteq A$ such that $|A'|\ge 0.99|A|$ and for any $u\in A'$ we have $N_{G}(u)\subseteq B$ and $|B-N_G(u)|\le a$, then the returned set $R$ satisfies $A'\subseteq R$ and $|N_G(u)\triangle N_G(v)|\le 5a$ for any $u,v\in R$.
    \end{itemize}
    The algorithm runs in time $O(\sum_{u\in A}|N_G(u)|)$.
\end{lemma}

\begin{proof}
    We first calculate $N_G(u)\cap A$ for any $u\in V$. This can be done by the following way in time $O(\sum_{u\in A}|N_G(u)|)$: for every $x\in A$, we increase the count for each $v\in N_G(x)$ by $1$. Now let $V'$ contain all $v$ with $|N_G(v)\cap A|\ge 0.1 |A|$. We claim that $V'\subseteq B$ and $|B-V'|\le 1.2a$. To see $V'\subseteq V$, notice that at most $0.01|A|$ nodes in $A$ have edges to $V-B$. To see $|B-V'|\le a$, notice that for a vertex in $B$ to be not included in $V'$, it needs to have more than $0.9|A|$ non-edges to $A$, which includes at least $0.89$ non-edges $A'$. However, the total number of non-edges from $A'$ to $B'$ is at most $a\cdot |A|$. Thus, there are at most $a\cdot |A|/0.9|A|\le 1.2a$ nodes in $B$ that is not in $V'$. Now we set $R$ to be all nodes $u\in A$ with $|N_G(u)\triangle V'|\le 2.2a$. For every node $u\in A'$, we have $|N_G(u)\triangle V'|\le a+1.2a\le 2.2a$, which means $A'\subseteq R$. For any $u,v\in R$, we have $|N_G(u)\triangle N_G(v)|\le 4.4a\le 5a$.

\end{proof}


\begin{algorithm}[H]
    \DontPrintSemicolon
    \caption{\textsc{TerminalReduction}$(G,T,k)$}
    \label{alg:terminalreduction}

    Let $(X,\mathcal{U})\leftarrow$\textsc{ExpanderDecomposition}$(G,T)$ (see~\cref{lem:vertexexpanderdecomposition})\;
    Let $S'=V,T_1=\emptyset,T_2=\emptyset$ and $T_3$ be arbitrary $\lfloor|T|/100\rfloor$ nodes in $T-X$\;\label{trlinet3}
    Let $\cU'=\{U\in\cU\mid 0<|T\cap U|<5\},\cU''=\{U\in\cU\mid |T\cap U|\ge 5\}$\;
    \ForEach{$U\in U''$}
    {Include arbitrary $\lceil\frac{2}{3}|T\cap U|\rceil$ vertices in $T\cap U$ into $T_1$\; \label{trlinet1}
    }
    Construct $G'=(X\cup\cU',E')$ where $E'=\{(x,U)\in X\times \cU'\mid \exists u\in U,(x,u)\in E\}$\; \label{trlineGp}
    Let $\cU'_{low}\leftarrow \{U\in\cU'\mid |N_{G'}(U)|\le 2k\}$ and $G'_{low}=G'[X\cup\cU'_{low}]$\;

    \ForEach{integer $1\le i\le \lceil\log k\rceil$\label{trlineloopi}}
    {
            Let $a\leftarrow 2^i$\;
            Let $X_{low}\leftarrow \{x\in X\mid |N_{G'_{low}}(x)|<1000a\}$\;
            \ForEach{$x\in X$}
            {
                Let $R_x\leftarrow$\textsc{Shaving}$(G'_{low},N_{G'_{low}}(x),a)$ (see~\cref{lem:shaving})\;\label{trlineshave}
                Let $H_x$ be the edge set of an arbitrary path on $R_x$\;\label{trlinepath}
            }
            Build a graph $G''$ with vertex set $\cU'_{low}$, and edge set be the union of $H_x$ for all $x\in X$\;\label{trlineGpp}
            Define distance function $\cAd(u,v)=|N_{G'}(u)\triangle N_{G'}(v)|$\;
            Let $\cP\leftarrow$\textsc{SNCConnected}$(G'',\cAd(u,v),15a)$ (see~\cref{lem:sparseneighborhoodcover})\;\label{trlinesnc}
            \ForEach{$P\in\cP$}
            {
                Let $X'\leftarrow X$\;
                \ForEach{$C\in P$}
                {
                    For arbitrary $\lfloor\frac{|C|}{\log^2 n}\rfloor$ nodes $U\in C\subseteq \cU'_{low}$, include $|T\cap U|$ into $T_2$\; \label{trlinet2}
                    \If{$|C|>10a\log^2n$}
                    {
                        \ForEach{$x\in X'\cap N_{G'}(C)$}
                        {Delete $x$ from $X'$ if $|N_{G'}(x)\cap C|>\left(1-\frac{1}{\log^3 n}\right)|C|$\;\label{trlinedelete}
                        }
                    }
                }
                Let $S_1\leftarrow$\textsc{BalancedTerminalVC}$(G,X'\cup T_3,k)$ (see~\cref{lem:balancedterminalalgorithm})\; \label{trlinex}
                Let $S_2\leftarrow$\textsc{BalancedTerminalVC}$(G,X_{low}\cup T_3,k)$\;\label{trlinexl}
                If $|S_1|<|S'|$, let $S'\leftarrow S_1$. If $|S_2|<|S'|$, let $S'\leftarrow S_2$\;
            }
    }
    Let $T'\leftarrow X\cup T_1\cup T_2\cup T_3$

    \Return $(S',T')$\;
\end{algorithm}

\subsection{Analysis (Proof of~\texorpdfstring{\cref{lem:terminalreduction}}{terminal reduction lemma})}
\label{subsec:tranalysis}

    \paragraph{Correctness.} We first show that $|T'|\le 0.9|T|$. Remember that $T'=X\cup T_1\cup T_2\cup T_3$. We bound each term as follows.
    \begin{enumerate}
        \item According to~\cref{lem:vertexexpanderdecomposition}, $|X|<0.01|T|$.
        \item According to~\cref{trlinet1}, $T_1$ includes $\lceil\frac{2}{3}|T\cap U|\rceil$ vertices for every $U$ with $T\cap U\ge 5$, which is at most $4|T\cap U|/5$ nodes. Remember that $U$ are disjoint for different $U\in\cU$, therefore, $|T_1|\le 4|T|/5$.
        \item According to~\cref{trlinet2}, we include $T\cap U$ into $T_2$ for at most $|C|/\log^2n$ number of $U$ for every $C\in\cC$. Since $|T\cap U|<5$, we includes at most $4|C|/\log^2n$ nodes into $T_2$ for each $C$. According to~\cref{lem:sparseneighborhoodcover}, $\sum_{C\in\cC}|C|=O(|\cU'_{low}|\log n)$. Since every $U\in \cU'$ contains at least one terminal in $T$, we have $|T_2|=O(|T|/\log n)$, which is at most $0.01|T|$ for sufficiently large $n$.
        \item According to~\cref{trlinet3}, we have $|T_3|\le 0.01|T|$.
    \end{enumerate}
    In total, $|T'|\le (0.01+0.8+0.01+0.01)|T|\le 0.9|T|$.

    It remains to prove either $S'$ is a minimum vertex cut of $G$ or $T'\subseteq V$ is a \strongbalanced{$0.01$} terminal set.
    Let $S$ be an arbitrary vertex cut of $G$ and $L$ be a connected component after deleting $S$ from $G$. Since $T$ is \strongbalanced{$2^{\sqrt{\log n}/2}$} and $k\in[\kappa_G,C\kappa_G]$ for sufficient large constant $C$, according to~\cref{def:balancedterminalset}, we have $|T\cap L|\ge 2^{\sqrt{\log n}/2}k$. Our goal is to prove that if $|T'\cap L|<0.01k$, then $S'$ (the output of~\cref{alg:terminalreduction}) must be a minimum vertex cut of $G$. Since $T'=X\cup T_1\cup T_2\cup T_3$, we can assume $|X\cap L|<0.01k$ and $|T_i\cap L|<0.01k$ for any $i$. Write $T_L=T\cap L,T_S=T\cap S,T_R=T\cap(V-L-S)$. In the following lemmas, we will specify what happens if $|T_i\cap L|<0.01k$ for each $i$, separately.

    \begin{lemma}\label{lem:T1}
        If $|X\cap L|<k/100$ and $|T_1\cap L|<k/100$, then $|\cup_{U\in\cU'}(T_L\cap U)|>2^{\sqrt{\log n}/2}k/4$.
    \end{lemma}
    \begin{proof}
        Suppose to the contrary, $|\cup_{U\in\cU'}(T_L\cap U)|\le 2^{\sqrt{\log n}/2}k/4$. Then we have $|\cup_{U\in\cU''}(T_L\cap U)|\ge 2^{\sqrt{\log n}/2}k/5$ since $|T_L|\ge 2^{\sqrt{\log n}/2}k$ and nodes in $T$ can be either $U\in\cU'\cup \cU''$ or $X$ where $|X|<0.01|T|$.

        Let $\tilde{\cU}$ contain all $U\in\cU''$ with (i) $|U\cap T_L|\ge |U\cap T_R|$, (ii) $|U\cap T_L|\ge 2|U\cap S|$. We first prove that $|\cup_{U\in\tilde{\cU}}(T_L\cap U)|\ge 2^{\sqrt{\log n}/2}k/10$. For that purpose, we will bound the size of $|\cup_{U\in\cU''-\tilde{\cU}}(T_L\cap U)|$. If (i) is violated, since $G[U]$ is a $(T,2^{-\log^{0.1}n})$-vertex expander according to~\cref{lem:vertexexpanderdecomposition} and according to the definition of expander~\cref{def:expander}, we have $\frac{U\cap S}{|U\cap (T_L\cup T_S)|}\ge 2^{-\log^{0.1}n}$ since $U\cap S$ is a vertex cut of $G[U]$. This gives us $|U\cap T_L|\le 2^{\log^{0.1}n}|U\cap S|$. Thus, the sum of $|U\cap T_L|$ for all $U$ violating (i) is at most $2^{\log^{0.1}n}k$. If (ii) is violated, then $U\cap T_L|<2|U\cap S|$. Thus, the sum of $|U\cap T_L|$ for all $U$ violating (ii) is at most $2k$. We get $|\cup_{U\in\tilde{\cU}}(T_L\cap U)|\ge 2^{\sqrt{\log n}/2}k/5-2^{\log^{0.1}n}k-2k\ge 2^{\sqrt{\log n}/2}k/10$.

        Notice that $U\cap T_L$ contains at least $0.4|U\cap T|$ nodes for $U\in\tilde{\cU}$ according to the above properties (i),(ii). According to~\cref{trlinet1}, we will include at least $2/3|T\cap U|$ many terminals in $T\cap U$ into $T_1$ for every $U\in\tilde{\cU}$, which contain at least $0.05|T\cap U|$ nodes from $T_L\cap U$. Since $|\cup_{U\in\tilde{\cU}}(T_L\cap U)|\ge 2^{\sqrt{\log n}/2}k/10$, we have $|T_1\cap L|\ge 0.05\cdot 2^{\sqrt{\log n}/2}k/10>k/100$, a contradiction.
    \end{proof}

    \begin{lemma}\label{lem:T2}
        If $|X\cap L|<k/100$ and $|T_1\cap L|,|T_2\cap L|<k/100$, then one of the following events happens.
        \begin{enumerate}
            \item There exists a loop~\cref{trlineloopi} such that $X_{low}$ in~\cref{trlinexl} satisfies $|X_{low}\cap S|=\tilde{O}(|X_{low}\cap L|)$ and $|T_3\cap S|=\tilde{O}(|X_{low}\cap L|)$.
            \item There exists a loop~\cref{trlineloopi} such that $X'$ in~\cref{trlinex} satisfies $|X'\cap S|=\tilde{O}(|X'\cap L|)$ and $|T_3\cap S|=\tilde{O}(|X'\cap L|)$.
        \end{enumerate}
    \end{lemma}
    \begin{proof}
        Let $\cU_{inside}\subseteq \cU'_{low}$ contain all $U$ such that $U\subseteq L$. Let $\cU_{cross}\subseteq \cU'_{low}$ contain all $U$ such that $U\cap (L\cup S)\not=\emptyset$ and $U\not\subseteq L$. Notice that for any $x\in X\cap L$, we have $N_{G'_{low}}(x)\subseteq \cU_{inside}\cup\cU_{cross}$.
        \begin{claim}
            $|\cU_{inside}|>k\log^9n$.
        \end{claim}
        \begin{proof}
            For any $U\in\cU'$, if $U\subseteq L$, then $|N_{G'}(U)|\le |X\cap L|+|S|\le 1.01k$ (that is because $S$ is a vertex cut), which implies $U\in\cU_{low}$. Also notice that for any $U\in\cU'$ with $T_L\cap U\not=\emptyset$, either $U\in\cU_{inside}$ or $U\cap S\not=\emptyset$ where the latter case can only happen for at most $k$ different $U$ as they are disjoint and $|S|\le k$. Each $U$ contain at most $4$ terminals in $T$, and due to~\cref{lem:T1}, we have $|\cup_{U\in\cU'}(T_L\cap U)|>2^{\sqrt{\log n}/2}k/4$, which means terminals inside $\cU_{inside}$ is at least $2^{\sqrt{\log n}/2}k/4-4k$, and $|\cU_{inside}|>2^{\sqrt{\log n}/2}k/16-k>k\log^9n$.
        \end{proof}

        We create $O(\log n)$ buckets for elements $U\in\cU_{inside}$ according to $|N_{G'}(U)\cap (X\cap L)|$. Let $\cU^j_{inside}$ contain all $U\in\cU_{inside}$ with $|N_{G'}(U)\cap (X\cap L)|\in [2^j,2^{j+1}]$. There exists $j$ such that $|\cU^j_{inside}|>k\log^8n$. Let $j$ be such an index and write $\cU^*=\cU^j_{inside}$. Consider the loop in~\cref{trlineloopi} when $2^i\in [2^{j-2},2^{j-1}]$. We write $a^*=2^i$.


        \begin{claim}\label{cla:xlow}
            In the loop $i$ described above, $|X_{low}\cap S|\le 16a^*$.
        \end{claim}
        \begin{proof}
            For every $U\in\cU^*$, we have $N_{G'}(U)\ge |S|$ and $|N_{G'}(U)\cap (X\cap L)|\le 8a^*$ and $N_{G'}(U)\subseteq (X\cap L)\cup(X\cap S)$. Thus, $|N_{G'}(U)\cap S|\ge |S|-8a^*$, in other words, $U$ has at most $8a^*$ non-edges to $S$. If $x\in X_{low}\cap S$, then it has at most $1000a^*$ edges to $\cU^*$, which is at most $1000k$. The number of non-edges from $x$ to $\cU^*$ is at least $|\cU^*|-1000k\ge |\cU^*|/2$. Thus, $|X_{low}\cap S|\le (8a^*|\cU^*|)/(|\cU^*/2)=16a^*$.
        \end{proof}
        We also need the following useful claim.
        \begin{claim}\label{cla:Ucross}
            $|U_{cross}|\le 8a^*$ and $|T_3|\le 8a^*$.
        \end{claim}
        \begin{proof}
            Take an arbitrary $U\in\cU^*$, we have $N_{G'}(U)\ge |S|$ and $N_{G'}(U)\cap L\le 8a^*$. Notice that $N_{G'}(U)\subseteq (L\cup S)\cap X$. Thus, $|N_{G'}(U)\cap S|\ge |S|-8a^*$, which implies $S-X\le 8a^*$. Each $U\in U_{cross}$ must contain at least one element in $S$, and they are disjoint. Remember that $T_3\subseteq T-X$. Therefore, $|U_{cross}|\le 8a^*$ and $|T_3|\le 8a^*$.
        \end{proof}
        Now if $|X_{low}\cap L|>0.01a^*$, according to~\cref{cla:xlow},\cref{cla:Ucross}, we have $|X_{low}\cap S|=\tilde{O}(|X_{low}\cap L|)$ and $|T_3\cap S|=\tilde{O}(|X_{low}\cap L|)$, which completes the proof. In what follows we assume $|X_{low}\cap L|\le 0.01a^*$. Write $X_{highL}=(X-X_{low})\cap L$ and $X_{lowL}=X_{low}\cap L$.

        We first define a graph on vertex set $X_{highL}$ where $x_1,x_2\in X_{highL}$ have an edge connecting them if $N_{G'}(x_1)\cap N_{G'}(x_2)\cap \cU_{inside}\not=\emptyset$. Suppose this graph has $\ell$ connected components denoted by $X_1,...,X_{\ell}$. We write $\cU_q=N_{G'_{low}}(X_q)\subseteq\cU_{inside}\cup\cU_{cross}$ and $\cU^{inside}_q=\cU_q\cap\cU_{inside}$.
        \begin{claim}\label{cla:cover}
            For any $q\in[\ell]$ with $|X_q|\ge a^*$, one of the loop of~\cref{trlineloopi} when $2^i$ (which we denote by $a$) satisfies $2|X_q|\le a< 4|X_q|$ (which must happen for exactly one $i$), there exists a partition $P\subseteq \cP$ (returned in~\cref{trlinesnc}) and a cluster $C\in P$ such that $\cU^{inside}_q\subseteq C$. Denote such partition as $P_q$ and such cluster as $C_q$.
        \end{claim}
        \begin{proof}
            Remember $R_x$ is defined in~\cref{trlineshave} for every $x\in X$. We first prove that for any $x\in X_q$, the condition described in~\cref{lem:shaving} is satisfied if we let $B=X_{lowL}\cup X_q\cup(X\cap S)$ and $A'=N_{G'_{low}}(x)\cap\cU_{inside}$. Notice that $A=N_{G'_{low}}(x)$ and $A-A'\subseteq \cU_{cross}$. According to~\cref{cla:Ucross}, we have $|A|-|A'|\le 8a^*$. Remember that $x\in X_q\subseteq X_{highL}$. According to the definition of $X_{highL}$, we have $N_{G'_{low}}(x)\ge 1000a^*$ (recall that the \emph{low}, \emph{high} is defined with respect to $a^*$), thus, $|A'|\ge 0.99|A|$. For any $U\in A'=N_{G'_{low}}(x)\cap\cU_{inside}$, we have $N_{G'}(U)\cap L\subseteq X_{lowL}\cup X_q$ since $X_q$ is a connected component where all neighbors of $N_{G'}(U)\cap X_{highL}$ should be in the same connected component $X_q$. Thus, $N_{G'}(U)\subseteq X_{lowL}\cup X_q\cup (X\cap S)=B$. Besides, we have $|N_{G'}(U)|\ge |S|$, which means $|B-N_{G'}(u)|\le |X_{lowL}|+|X_q|+|S|-|S|\le 0.01a^*+0.5a\le 0.51a$. Thus, all conditions are satisfied~\cref{trlineshave}. The conclusion we get is: $R_x$ satisfies $N_{G'_{low}}(x)\cap\cU_{inside}\subseteq R_x$ and $|N_{G'}(u)\triangle N_{G'}(v)|\le 5a$ for any $u,v\in R_x$.

            Write $R_q=\cup_{x\in X_q}R_x$. We will prove that (i) $\cU^{inside}_q\subseteq R_q$, (ii) $G''[R_q]$ is connected, (iii) $|N_{G'}(u)\triangle N_{G'}(v)|\le 15a$ for any $u,v\in R_q$. If all of them are correct, then according to~\cref{lem:sparseneighborhoodcover} property (cover), there exists $C\in P\in \cP$ such that $\cU^{inside}_q\subseteq R_q\subseteq C$ and the proof is finished.

            \paragraph{(i) $\cU^{inside}_q\subseteq R_q$.} This follows from $N_{G'_{low}}(x)\cap\cU_{inside}\subseteq R_x$ for any $x\in X_q$ and $\cU^{inside}_q=\cU_q\cap\cU_{inside}$.

            \paragraph{(ii) $G''[R_q]$ is connected.} Remember that in $G''$, there is a path on $R_x$ for every $x\in X_q$. Recall that $X_q$ is connected in the sense that $x,y\in X_q$ have an edge if they share a neighbor in $\cU_{inside}$, in which case the path $R_x,R_y$ are connected together since $N_{G'_{low}}(x)\cap\cU_{inside}\subseteq R_x$ for any $x\in X_q$. Therefore, $G''[R_q]$ (which is the union of paths $R_x$ for $x\in X_q$) is connected.

            \paragraph{(iii)$|N_{G'}(u)\triangle N_{G'}(v)|\le 15a$ for any $u,v\in R_q$.} For any $u\in\cU^{inside}_{q}$, we have $N_{G'}(u)\subseteq X_{lowL}\cup X_q\cup S$ and $|N_{G'}(u)|\ge |S|$, which implies $|N_{G'}(u)\triangle N_{G'}(v)|\le 2|X_{lowL}\cup X_q\cup S|-|S|-|S|\le 1.02a$. For any $w\in R_q-\cU^{inside}_q$, there exists $u\in \cU^{inside}_q$ such that they are in the same path $R_x$ for some $x\in X_q$ and $|N_{G'}(u)\triangle N_{G'}(w)|\le 5a$. Thus, according to the triangle inequality for symmetric difference, we have $|N_{G'}(u)\triangle N_{G'}(v)|\le 15a$ for any $u,v\in R_q$.
        \end{proof}

        Now we have $P_q$ and $C_q$ for every $q\in[\ell]$ with $|X_q|\ge a^*$ and $\cU^{inside}_q\subseteq C_q$, we have the following claim.
        \begin{claim}
            There exists $q\in[\ell]$ with $|X_q|\ge a^*$ and $|C_q|\ge (\log^4n)|X_q|$ where $|\cU^{inside}_q|< (1-1/2\log^2 n)|C_q|$.
        \end{claim}
        \begin{proof}
            If to the contrary, $|\cU^{inside}_q|\ge (1-1/2\log^2 n)|C_q|$ holds for any of them, then according to~\cref{trlinet2}, at least $|\cU^{inside}_q|/2\log^2 n$ nodes in $T\cap L$ is included in $T_2$. If we can prove $\sum_{|X_q|\ge a^*}|\cU^{inside}_q|\ge k\log^5n$, then $\sum_{|X_q|\ge a^*,|C_q|\ge(\log^4n)|X_q|}|\cU^{inside}_q|\ge k\log^5n-\sum_{q}(\log^4n)|X_q|\ge k\log^5n-0.01k\log^4n$, violating the fact that $|T_2|<0.01k$. Remember that $|\cU^*|\ge k\log^8n$ where $\cU^*$ only contain $U\in\cU_{inside}$ with $|N_{G'}(U)\cap (X\cap L)|\ge 2a^*$. Any $U\in\cU^*$ satisfies $N_{G'}(U)\cap (X\cap L)\subseteq X_{lowL}\cup X_{highL}$ where the part in $X_{lowL}$ has size at most $0.01a^*$, and the part in $X_{highL}$ must be in the same $X_q$ for some $q$, implying $|X_q|\ge 1.99a^*$. Thus, $\sum_{|X_q|\ge a^*}|\cU^{inside}_q|\ge k\log^5n$.
        \end{proof}


        Now we have $q\in[\ell]$ with $|X_q|\ge a^*$ and $|C_q|\ge (\log^4n)|X_q|$ where $|\cU^{inside}_q|< (1-1/2\log^2 n)|C_q|$. We will prove that $X'$ (in~\cref{trlinex}) satisfies $|X'\cap S|=\tilde{O}(|X'\cap L|)$ in this specific loop when $P=P_q$, which finishes the proof. We first show that $X_q\subseteq X'$, i.e.,~\cref{trlinedelete} does not delete any vertex in $X_q$. This is because for any $x\in X_q$, $N_{G'}(x)\subseteq \cU^{inside}_q\cup \cU_{cross}$ where $|\cU^{inside}_q|< (1-1/2\log^2 n)|C_q|$ and $|\cU_{cross}|\le 8a^*\le 8|X_q|\le |C_q|/\log^4n$. It remains to prove $|X'\cap S|=\tilde{O}(|X_q|)=O(|X'\cap L|)$. Let $u\in\cU^{inside}_q$ be an arbitrary element. We have $|N_{G'}(u)\cap S|\ge |S|-|X_{lowL}|-|X_q|\ge |S|-0.1a$ (remember that $|X_q|\ge a/4$ and $a\ge a^*$). Notice that for any $v\in C_q$, we have $|N_{G'}(u)\triangle N_{G'}(v)|=O(a\log n)$ according to~\cref{lem:sparseneighborhoodcover} property (low diameter). Thus, we have $|N_{G'}(v)\cap S|\ge |S|-O(a\log n)$ for any $v\in C_q$. For a vertex $s\in S$ to not be deleted, it needs to have at least $|C_q|/\log^3n$ many non-edges to $C_q$. However, there are at most $O(a\log n)|C_q|$ many non-edges from $C_q$ to $S$. Thus, the number of nodes in $S$ that is not deleted is at most $O(a\log n)|C_q|/(|C_q|/\log^3n)=\tilde{O}(a)=\tilde{O}(|X_q|)=O(|X'\cap L|)$. Besides, according to~\cref{cla:Ucross}, we have $|T_3\cap S|=O(a^*)=O(|X'\cap L|)$, which finishes the proof.






















    \end{proof}

    With~\cref{lem:T2}, further assume $|T_3\cap L|<k/100$ (otherwise we are done), the $S_1$ in~\cref{trlinex} or $S_2$ in~\cref{trlinexl} will be a minimum vertex cut of $G$: $|(X'\cup T_3)\cap S|=\tilde{O}(X'\cap L)$ holds due to~\cref{lem:T2}, $|(X'\cup T_3)\cap L|\le 0.02k$ due to $|X\cap L|<0.01k$ and $|T_3\cap L|<0.01k$, $|T_3\cap (V-L-S)|>k$ due to $|T-X|>(\log n)k$ and $|T_3|\ge |T|/101$, similar for $X_{low}$.


    \paragraph{Complexity.} One can verify that most lines of the algorithm can be run in time $\hat{O}(mk)$. We will explain some non-trivial parts as follows.
    \begin{enumerate}
        \item \textbf{Construction of auxiliary graphs.} $G'$ is constructed by first deleting all vertex set in $\cU''$ from $G$, and then contract every vertex set in $\cU'$. $G'_{low}$ is an induced subgraph of $G'$.

        \item \textbf{Call of Shaving.} In~\cref{trlineshave}, the total running time according to~\cref{lem:shaving} is $\sum_{x\in X}\sum_{U\in N_{G'_{low}}(x)}|N_{G'}(U)|$. Here $|N_{G'}(U)|\le 2k$ since $U\in\cU'_{low}$. Thus, it is at most $k\sum_{x\in X}|N_{G'_{low}}(x)|=O(km)$ since the number of edges in $G'_{low}$ is at most $m$.

        \item \textbf{Size of $G''$ and call of SNCConnected.} $G''$ is a union of path $H_x$, where $H_x$ is a path with length at most $|N_{G'_{low}}(x)|$. Thus, the number of edges in $G''$ is at most $m$. Moreover, the maximum degree is at most $4k$ since for every $u\in\cU'_{low}$, we have $|N_{G'}(u)|\le 2k$, where each $x\in N_{G'}(u)$ will add at most $2$ edges to $u$ in $G''$.
        The distance oracle $\cA_{dist}(u,v)$ for any $u,v\in \cU'_{low}$ (which is the vertex set of $G''$) can be computed in time $O(k)$ since $|N_{G'}(u)|,|N_{G'}(u)|\le 2k$ according to the definition of $\cU'_{low}$. Therefore, according to~\cref{lem:sparseneighborhoodcover}, the running time for the \textsc{SNCConnected} call is at most $\tilde{O}(mk)$.

        \item \textbf{Delete vertex from $X'$.} The size $\cP$ is at most $O(\log n)$ according to~\cref{lem:sparseneighborhoodcover}, where each $P\in\cP$ is a partition. Now we explain the total running time of~\cref{trlinedelete}. To implement it for a specific $P\in\cP$, we first iterate over all $x\in X$ and $u\in N_{G'_{low}}(x)$, add a count $1$ to the $C\in P$ for $u\in C$, which cost $O(m)$ time. After that, we get $|N_{G'_{low}}(x)\cap C|$ for every $x\in X$ and $C\in P$. For each $C$, we can find $N_{G'}(C)$ in time the sum of the degree of every node in $C$, and decide whether to delete each node or not in $O(1)$ time. Since $P$ is a partition, it costs time $O(m)$.
    \end{enumerate}



==> unbalanced.tex <==

\section{\texorpdfstring{An $\widehat{O}(m \kappa)$}{Ohat(mk)}-Time Vertex Connectivity Algorithm for Unweighted Undirected Graphs}
\label{sec:Algorithmunweighted}

In this section, we will prove the following lemma.  Throughout this section, $\delta$ is the minimum degree of the input graph. We can view $\delta$ as a constant approximation of the vertex connectivity of the graph by standard sparsification techniques~\cite{NagamochiI92}.

\begin{lemma}\label{lem:unbalanced}
    There is a deterministic algorithm that takes inputs an $n$-nodes $m$-edges undirected graph $G=(V,E)$, and outputs a vertex cut of $G$. If there exists a minimum vertex cut $(L,S,R)$ of $G$ satisfying $|L|= O(\delta)$ and $|L| \leq |R|$, then the output is a minimum vertex cut of $G$. The algorithm runs in  $\widehat{O}(m\delta)$ time.
\end{lemma}


To prove~\cref{lem:unbalanced}, we will use the following lemma, which is proved in~\cref{subsec:lemmadatastructure}.

\newcommand{\tka}{\tilde{\kappa}}
\begin{lemma}\label{lem:datastructure}
There is a deterministic algorithm that, given an undirected graph $G$ and an integer $\ell$, in $\widehat{O}(m\delta)$ time returns
\begin{enumerate}
    \item vertex sets $V_{1},\dots,V_{z}$ where each vertex $v\in V$ is contained in at most $O(\log n)$ many $V_i$ for different $i$,
    \item a data structure $\cD$ that, given any vertices $s$ and $t$, it returns an integer $\tka\ge\kappa(s,t)$ in $\hO{\delta \ell}$ time.
\end{enumerate}

Suppose $(L,S,R)$ is a minimum vertex cut of $G$. If $|L|\le |R|$ and $\ell=[|L|,2|L|]$, then one of the following two events happens.

\begin{enumerate}
    \item $\exists i,L\subseteq V_i,|V_i\cap S|=\tilde{O}(|L|),|V_i\cap R|=\tilde{\Omega}(|L|)$.
    \item If $\cD$ is given $s\in L,t\in R$, it will return $\tka=\kappa(G)$.
\end{enumerate}
\end{lemma}

Next, we show how to use~\cref{lem:datastructure} to prove~\cref{lem:unbalanced}.


\begin{proof}[Proof of~\cref{lem:unbalanced}]
   We describe an algorithm and analysis.
   \paragraph{Algorithm.}  For every $\ell=2^i$ from $i=1$ to $i=\lceil\log (\delta\log n)\rceil$ (which serves as an estimate of $|L|$), the algorithm uses the following procedure (called the $i$-th iteration) to find the separator $S^{(i)}$ as follows.

    The algorithm firstly uses \cref{thm:crossing family} with parameters $\alpha = \frac{2\delta}{\ell}$ to compute an $(n,\alpha)$-crossing family $P$. Then, it uses   \cref{lem:datastructure} on $G,\ell$ to get (i) $V_1,V_2,...,V_z$, (ii) the data structure $\cD$. Then the algorithm uses~\cref{lem:subgraphbalancedterminalalgorithm} on $G,V_i,\delta\log n$ for every $i\in[z]$ to get separators $S_1,...,S_z$, and uses the data structure $\cD$ with queries $(s,t)\in P$ to get $\tka_{s,t}\ge \kappa(s,t)$ for every $(s,t)\in P$.
     If among $|S_1|,...,|S_z|$ and $\tka_{s,t}$ for any $s,t\in P$, the minimum value is $|S_i|$, then set $S^{(i)}=S_i$; otherwise, suppose the minimum value is $\tka_{s,t}$ for some $(s,t)\in P$, we set $S^{(i)}$ to be the minimum separator between $s,t$, denoted by $S_{s,t}$, which can be found by one call to vertex-capacity max flow.

     Finally,  return the minimum $S^{(i)}$ among all $i$ as the output.






    \paragraph{Correctness.} According to~\cref{lem:subgraphbalancedterminalalgorithm}, the returned cuts $S_1,...,S_z$ are always a valid separator. Besides, $S_{s,t}$ must be a valid separator since it is deduced from a vertex-capacity max flow from $s$ to $t$. Thus, we just need to prove that one of $S^{(i)}$ is a minimum separator. Suppose $(L,S,R)$ is one of the minimum separators of $G$ with $|L|\le |R|$ and $|L|,|S|=O(\delta)$. There must exist $i$ such that $\ell=2^i\in[|L|, 2|L|]$. We will prove that $S^{(i)}$ is a minimum cut. In order to prove this, we just need to show that in the $i$-th iteration, either one of $S_1,...,S_z$ is a minimum cut, or one of $\tka_{s,t}$ for $(s,t)\in P$ satisfies $\tka_{s,t}=\kappa(G)$. If this is true, then $S^{(i)}$ is either $|S_j|$ for some $j$ such that $|S_j|=\kappa(G)$, or some $s,t$ minimum separator for some $(s,t)\in P$ with $\tka_{s,t}=\kappa(G)\ge \kappa(s,t)$ (in which case $\kappa(s,t)=\kappa(G)$).


    According to~\cref{lem:datastructure}, there are two events to consider.

    \textbf{Case 1: $\exists i,L\subseteq V_i,|V_i\cap S|=\tilde{O}(|L|),|V_i\cap R|=\tilde{\Omega}(|L|)$.} In this case, since $|V_i\cap L|\le |L|\le \delta\log n$, by using~\cref{lem:subgraphbalancedterminalalgorithm} on $G,V_i,\delta\log n$, we can get $S_i$ which is a minimum separator of $G$.

    \textbf{Case 2: $\cD$ is given $s\in L,t\in R$.} We prove that it will return $\tka=\kappa(G)$. Indeed,

    \begin{lemma}\label{lem:stinP}
        there exists $(s,t)\in P$ such that $s\in L,t\in R$.
    \end{lemma}

    \begin{proof}
        Let $(L,S,R)$ be a vertex mincut in $G$ where $|R| \geq |L|$.
        Since $S$ is a minimum separator, $|S|\le \delta$ (otherwise the neighborhoods of the vertex with a minimum degree should be the minimum separator). We have $|S|/|L|\le (\delta)/(\ell/2) = \alpha$. According to~\cref{thm:crossing family}, since we have $|R| \geq |L| \geq |S|/\alpha$, there exists $(s,t)\in P$ such that $s\in L,t\in R$.
    \end{proof}

    By~\cref{lem:datastructure}, $\cD$ will return $\tka_{s,t}=\kappa(G)$ on such $s\in L,t\in R$.

    \paragraph{Time complexity.} For each iteration, \cref{thm:crossing family,lem:datastructure} use $\tO{m\delta}$ time. Then \cref{lem:subgraphbalancedterminalalgorithm} on each $V_i$ takes time $\hO{\sum_{v\in V_i}|N_{G}(v)|}$, which in total takes time $\hO{m\delta}$ since each vertex in $V$ is included in at most $O(\log n)$ $V_i$'s. One call to $s,t$ vertex-capacity max flow takes time $\hO{m}$. It remains to bound the running time of queries to $\cD$, which is
    \[ |P| \cdot \widehat{O}( \delta \ell) = O(n \alpha) \cdot \widehat{O}( \delta \ell) = \widehat{O}( n \delta^2) = \widehat{O}( m \delta).\]
The first equality follows from \cref{thm:crossing family,lem:datastructure}.
\end{proof}


\subsection{Sparse Neighborhood Cover Algorithm}\label{sec:sparseneighborhoodcover}

Before proving~\cref{lem:datastructure}, we first need to introduce a fast algorithm for computing sparse neighborhood cover for our purpose.

\begin{lemma}\label{lem:sparseneighborhoodcover}
    There is a deterministic algorithm \textsc{SNCConnected}$(G,\cAd,d)$ (\cref{alg:snc}) that takes as inputs an $n$-vertex $m$-edge undirected graph $G=(V,E)$, a symmetric distance oracle $\cAd:V\times V\to \bbN$ and $d\in\bbN^+$ which satisfies triangle inequality $\cAd(u,v)+\cAd(v,w)\ge \cAd(u,w)$, outputs a set of partitions of $V$ denoted by $\cP$ such that
    \begin{enumerate}
        \item (sparse) $|\cP|=O(\log n)$, for every $P\in\cP$, $P\subseteq 2^V$ is a partition of $V$, which means $\cup_{C\in P}C=V$ and $C_1\cap C_2=\emptyset$ for $C_1,C_2\in P$ with $C_1\not=C_2$, we call $C$ a \emph{cluster},
        \item (cover) for any $L\subseteq V$ where $G[L]$ is connected and $\cAd(u,v)\le d$ for any $u,v\in L\cap U$, there exists a cluster $C$ such that $L\subseteq C$,
        \item (low diameter) for any cluster $C$, for any $u,v\in C$, we have $\cAd(u,v)=O(d\log n)$.
    \end{enumerate}
    The algorithm uses $\tO{m}$ calls to $\cAd$ and in addition $\tilde{O}(n\max_{v\in V}|N_G(v)|)$ time.
\end{lemma}




\begin{algorithm}[H]
    \DontPrintSemicolon
    \caption{\textsc{SNCConnected}$(G,\cAd,d)$}
    \label{alg:snc}
    Let $\cP\leftarrow \emptyset$\;
    Let $G'=(V,H=\{(u,v)\in E\mid \cAd(u,v)\le d\})$\;
    \While{$U\not=\emptyset$\label{snclinewhile1}}
    {
        Let $\cC\leftarrow \emptyset$\;
        Let $U_{rem}\leftarrow U,U_{next}\leftarrow \emptyset$\;
        \While{$U_{rem}\not=\emptyset$\label{snclinewhile2}}
        {
            Let $u$ be an arbitrary node in $U_{rem}$\;
            Let $T_0\leftarrow \emptyset,T_1=\{u\},i=1$\;
            \While{$|N_{G'[U_{rem}]}(T_i)|\ge |T_{i-1}|$ or $|T_i|\ge 1.1|T_{i-1}|$\label{snclinewhile3}}
            {
                $i\leftarrow i+1$\;
                Build BFS tree $T_{i}$ on $G'[U_{rem}]$ with root $u$ and only include $v$ to $T$ if $\cAd(u,v)\le 5id$\label{snclineTi}\;
            }
            Build BFS tree $T$ on $G'[U_{rem}]$ with root $u$ and only include $v$ to $T$ if $\cAd(u,v)\le (5i-3)d$\label{snclineTB}\;
            Let $\cC=\cC\cup\{T\}$\label{snclineT}\;
            Let $U_{rem}\leftarrow U_{rem}-T$\label{snclinerem}\;
            Let $U_{next}\leftarrow U_{next}\cup (T_i-T_{i-1})$\label{snclineU}\;
        }
        $U\leftarrow U_{next}$\;
        $\cP\leftarrow\cP\cup\{\cC\}$
    }
    \Return{$\cP$}
\end{algorithm}

\begin{proof}[Proof of~\cref{lem:sparseneighborhoodcover}]
    We first prove \emph{(sparse)}. Notice that in the same while loop (\cref{snclinewhile2}), the tree nodes included in $\cC$ (\cref{snclineT}) are disjoint since~\cref{snclineTB} creates $T$ on $G'[U_{rem}]$ where $T$ is deleted from $U_{rem}$ (\cref{snclinerem}). They form a partition of $V$ since the loop ends if $U_{rem}=\emptyset$. Thus, we only need to prove that the outer while loop (\cref{snclinewhile1}) only contains $O(\log n)$ loops. We will prove that in each loop, $|U_{next}|\le 0.1|U|$, which implies the $O(\log n)$ loop numbers since we set $U\leftarrow U_{next}$ at the end of each loop. Notice that $U_{next}$ includes $T_i-T_{i-1}$ (\cref{snclineU}) where $T_{i-1}\subseteq T$ which is deleted from $U_{rem}$, and from the condition of~\Cref{snclinewhile3} we have $|T_{i}|<1.1|T_{i-1}|$ which implies $|T_i-T_{i-1}|\le 0.1|T|$. Thus, we can charge $|T_i-T_{i-1}|$ into $0.1|T|$. Notice that the sum of all $|T|$ is at most $|U|$ (\cref{snclinerem}), we have $|U_{next}|\le 0.1|U|$.

    Next, we prove \emph{(cover)}. Suppose $L\subseteq V$ where $G[L]$ is connected and $\cAd(u,v)\le d$ for any $u,v\in L$. We will prove that there exists $C\in\cC\in\cP$ such that $L\subseteq C$. For this purpose, we only need to prove the following loop invariance: in the while loop~\cref{snclinewhile1}, if $L\subseteq U$ in the beginning, then at the end of this loop, either there exists $C\in\cC$ such that $L\subseteq C$ or $L\subseteq U_{next}$. Since $U_{next}$ will be $U$ in the next loop, the loop invariance will imply \emph{(cover)}. Now suppose $L\subseteq U$. Notice that the trees $T$ included in $\cC$ (\cref{snclineT}) in this while loop form a partition of $U$, there must exist $T$ such that $L\cap T\not=\emptyset$. Let $T$ be the first one in the loop of~\cref{snclinewhile2} that $L\cap T\not=\emptyset$ (which means $L\subseteq U_{rem}$ at this point). If $L\subseteq T$ then we are done since $T$ is included in $\cC$. Suppose $L\not\subseteq T$, we claim that $L\cap T_{i-1}=\emptyset$. Otherwise, there exists $w\in L\cap T_{i-1}$ such that $\cAd(u,w)\le (5i-5)d$, which implies $\cAd(u,v)\le (5i-4)d$ for any $v\in L$. Also notice that for any edge $(u,v)\in G[L]$ we have $\cAd(u,v)\le d$, thus, $(u,v)\in H$ and $G[L]=G'[L]$ which is connected. Thus, we get $L\subseteq T$ since $T$ is a BFS tree that includes a node $v$ if $v\in N_{G'[U_{rem}]}(T)$ and $\cAd(u,v)\le (5i-3)d$ (\cref{snclineTB}), a contradiction. Now we have $L\cap T_{i-1}=\emptyset$. Let $w\in L\cap T$, we have $\cAd(u,w)\le (5i-3)d$ and $\cAd(u,v)\le d$ for any $v\in L$, which implies $\cAd(u,v)\le (5i-2)d$ for any $v\in L$.  Therefore, $L\subseteq T_i$ since $T_i$ is a BFS tree with root $u$ which includes all nodes $v$ with $\cAd(u,v)\le 5id$. Therefore, $L\subseteq T_i-T_{i-1}$, which means $L\subseteq U_{next}$.

    Next, we prove \emph{(low diameter)}. This is because $\cC$ only includes $T$ where $T$ contains all nodes $v$ satisfying $\cAd(u,v)\le (5i-3)d$ for a specific node $v$. If we can prove that $i=O(\log n)$, then we are done. For that purpose, we need to prove the while loop~\cref{snclinewhile3} only contains $O(\log n)$ loops. There are two cases for the while loop to continue. One is $|T_i|\ge 1.1|T_{i-1}|$, which can happen at most $O(\log n)$ times since $|T_i|\le n$ for any $i$. In the case that $|N_{G'[U_{rem}]}(T_i)|\ge |T_{i-1}|$, we will prove that $|T_{i+1}|\ge 1.1|T_{i}|$. For every vertex $v\in N_{G'[U_{rem}]}(T_i)$, there exists $w\in T_i$ such that $(w,v)\in H$, which means $\cAd(w,v)\le d$, thus, $\cAd(u,v)\le \cAd(w,v)+\cAd(u,w)\le 5(i+1)d$ and $v\in T_{i+1}$. In other words, each loop of~\cref{snclinewhile3} implies that $|T_{i+1}|\ge 1.1|T_{i-1}|$, which can happen at most $O(\log n)$ times.

    Next, we prove the running time. To construct $G'$, we need $m$ calls to $\cAd$ and $O(m)$ running time. As proven above, there are at most $O(\log n)$ loops of~\cref{snclinewhile1}. In each loop, as proven above, there are at most $O(\log n)$ loops of~\cref{snclinewhile3}. Each of them builds a BFS tree with root $u$, while building the tree $T_i$ will cost $|T_i\cup N_{G'[U_{rem}]}(T_i)|$ many $\cAd$ calls (since we calculate the distance of each of them with $u$) and in addition the number of edges inside $T_i\cup N_{G'[U_{rem}]}(T_i)$ time, which is at most $|T_i\cup N_{G'[U_{rem}]}(T_i)|\cdot \max_{v\in V}|N_{G'}(v)|$. Notice that $T_{i-1}$ is deleted from $U_{rem}$ and $|T_i\cup N_{G'[U_{rem}]}(T_i)|=O(|T_{i-1}|)$ at the end of loop~\cref{snclinewhile3}. Thus, we can charge the oracles and running time to $\tilde{O}(T_{i-1})$. Since $|U_{rem}|\le n$, the number of oracles is bounded by $\tilde{O}(n)$ and the running time is bounded by $\tilde{O}(n\max_{v\in V}|N_{G}(v)|)$.
\end{proof}

\subsection{Proof of \texorpdfstring{\cref{lem:datastructure}}{data structure lemma}}
\label{subsec:lemmadatastructure}

We need the following sparse recovery tool from~\cite{NanongkaiS17}.

\begin{lemma}[Deterministic sparse recovery, corollary of Theorem 4.14~\cite{NanongkaiS17}]\label{lem:sparserecovery}
    There are deterministic algorithms $\cA_{construct}(G,x)$ and $\cA_{recover}(\vec{v},\vec{u})$ such that
    \begin{itemize}
        \item $\cA_{construct}$ takes as inputs an undirected graph $G=(V,E)$ and a positive integer $x$  outputs a vector $\vec{v}$ with length $\hat{O}(x)$ for each $v\in V$ in $\hat{O}(m)$ time,
        \item $\cA_{recover}$ takes as inputs two vectors $\vec{v},\vec{u}$ computed by $\cA_{construct}$, outputs $N_G(u)\triangle N_G(v)$ in $\hat{O}(x)$ time if $|N_G(u)\triangle N_G(v)|\le x$.
    \end{itemize}
\end{lemma}

\begin{proof}
    In Theorem 4.14~\cite{NanongkaiS17}, we set $k=x$ and $n=|V|$, we can construct $\Phi\in\{0,1\}^{d\times n}$ ($d=\hat{O}(x)$) implicitly in $\hat{O}(n)$ time by knowing all the non-zero entities. Now we define $\vec{N_G(u)}\in\{0,1\}^n$ for each $u$ to be the identity vecter where the $i$-th entry is $1$ iff. the $i$-th node in $V$ is in $N_G(u)$. $\cA_{construct}$ will output $\vec{v}=\Phi\vec{N_G(u)}$ for any $u\in V$, which takes time $\hat{O}(m)$ in total since $\Phi\vec{N_G(u)}$ takes time $\hat{O}(|N_G(u)|)$ (each column of $\Phi$ has $\hat{O}(1)$ non-zero entries).

    $\cA_{recover}$ will take $\Phi\vec{N_G(u)},\Phi\vec{N_G(v)}\in\{0,1\}^d$ and compute $\Phi(\vec{N_G(u)}-\vec{N_G(v)})$. According to Theorem 4.14~\cite{NanongkaiS17}, if $\vec{N_G(u)}-\vec{N_G(v)}$ contains at most $x$ non-zero entries (i.e., $|N_G(u)\triangle N_G(v)|\le x$), then all the non-zero entries are returned, which give us $N_G(u)\triangle N_G(v)$.
\end{proof}

We show our algorithm for~\cref{lem:datastructure} as follows, i.e., how to compute the vertex sets $V,V_1,...,V_z$ and the memory space of the data structure $\cD$. We will show how $\cD$ uses the memory space to answer a query later.

\paragraph{Algorithm for~\cref{lem:datastructure}.} The algorithm takes inputs an undirected graph $G = (V,E)$ and an integer $\ell$. The following procedure will find the data structure $\cD$.

\newcommand{\Visize}{O(\delta\log n)}

\begin{enumerate}
    \item Compute the minimum degree of the graph, denoted by $\delta$. Compute $V-N_{G}(v)$ for any $v\in V$. Let $V_{low}$ contain all vertices $v$ with $|N_G(v)|=O(\delta)$.
    \item Define distance $\cAd(u,v)$ for any $u,v\in V_{low}$ as $\cAd(u,v)=|N_G(u)\triangle N_G(v)|$. Notice that $\cAd(u,v)$ can be computed in time $\tilde{O}(\delta)$.
    \item Let $\cP\leftarrow$\textsc{SNCConnected}$(G[V_{low}],\cAd,4\ell)$, Let $V_1,...,V_z$ be all vertex sets in $\cC$ for all $\cC\in\cP$, i.e., $z=\sum_{\cC\in\cP}|\cC|$.
    \item Use $\cA_{construct}(G,\ell\log^2n)$ in~\cref{lem:sparserecovery} to get a vector $\vec{v}$ for any $v\in V$.
    \item Data structure $\cD$ memorizes (i) $V_1,...,V_z$ and the sizes of them, (ii) for any $u\in V$, the index set $I_u=\{i\mid u\in V_i\}$, (iii) the vectors $\vec{v}$ for any $v\in V$, (iv) $V-N_{G}(v)$ for any $v\in V$.
\end{enumerate}

The algorithm returns vertex sets $V,V_1,...,V_z$ and the data structure $\cD$. We will show the query algorithm for $\cD$ later. The following claim is a crucial property.

\begin{claim}\label{cla:nearneighbor}
    For every $u,v\in V_i$, $|N_G(u)\triangle N_G(v)|=O(\ell\log n)$.
\end{claim}
\begin{proof}
    From~\cref{lem:sparseneighborhoodcover}, we have $\cAd(u,v)=O(\ell\log n)$. According to the definition of $\cAd$, we have $|N_G(u)\triangle N_G(v)|=O(\ell\log n)$.
\end{proof}

The following lemma shows the running time of the algorithm.

\begin{lemma}\label{lem:constrcuttime}
    The algorithm for constructing vertex sets and $\cD$ described above runs in time $\tO{m\delta}$.
\end{lemma}
\begin{proof}
    We analyze each step.
    \begin{enumerate}
        \item Computing the minimum degree and $V-N_{G}(v)$ for all $v$ costs $O(m)$.
        \item The distance oracle uses time $\tilde{O}(\delta)$ for each query.
        \item By~\cref{lem:sparseneighborhoodcover}, the running time is $\tilde{O}(m\delta)$.
        \item By~\cref{lem:sparserecovery}, the running time is $\hat{O}(m)$.
    \end{enumerate}
\end{proof}
\paragraph{Query algorithm for the data structure $\cD$.} Before stating our algorithm, we first define our \emph{kernel graph} with respect to some $V_i$ and $s\in V_i,t\in V$ as follows.


\newcommand{\Vist}{V^i_{s,t}}
\newcommand{\Eist}{E^i_{s,t}}
\newcommand{\Gist}{G^i_{s,t}}

\begin{definition}\label{def:gist}
    For $i\in [z],s\in V_i,t\in V$, let $V'_i=V_i\setminus N_G[t]$, define $\Gist=(\Vist,\Eist)$ where
    \begin{align*}
    \Vist= & N_G[V'_i]\cup\{t\}\\
        \Eist= & \{(s,v)\mid v\in N_G(s)\} \\
    &\cup\{(u,v)\mid u\in V'_i,v \in N_G(u) \setminus N_G(s)\}\\
    &\cup \{(u,t)\mid u\in N_G(V'_i), u\not=t\}
    \end{align*}

\end{definition}


Note that the construction of $G_{s,t}^i$ is the same as the one described in the overview. We state the following key properties of $G_{s,t}^i$ whose proofs are essentially the same as shown in the overview. We omit for brevity.

\begin{lemma}\label{lem:atleastkappaG}
     $\kappa_{\Gist}(s,t) \geq \kappa_G(s,t)$.
\end{lemma}

\begin{lemma}\label{lem:whensinLtinR}
    Let $(L,S,R)$ be a minimum vertex cut of $G$. If  $s\in L,t\in R, L\subseteq V_i$, then
    $\kappa_{\Gist}(s,t) = \kappa(G)$.
\end{lemma}

Now we are ready to state our query algorithm for $\cD$.

	\par\addvspace{.5\baselineskip}
	\framebox[16cm][l]{
		\noindent
		\parbox{15.5cm}{
			\par\addvspace{.2\baselineskip}
			\hypertarget{alg:static}{\underline{\emph{Query Algorithm for $\cD$}}}
			\par\addvspace{.3\baselineskip}
			\begin{enumerate}
			    \item Let $I_s$ be all index $i$ with $s\in V_i$. If $I_s=\emptyset$, \textbf{return} $n$.
                    \item   $I'_s=\{i\in I_s\colon |V_i|\le\Visize\}$. If $I'_s=\emptyset$, \textbf{return} $n$.
                    \item For every $i\in I'_s$, construct a graph $\Gist=(\Vist,\Eist)$ defined in~\cref{def:gist}.

                    \item Let $S'$ be the minimum $(s,t)$-separator in $\Gist$ (which can be done by solving a vertex-capacity max flow on $\Gist$).
                    \item \textbf{return} $|S'|$.

			\end{enumerate}
			\par\addvspace{.2\baselineskip}

		}
	}
	\par\addvspace{.5\baselineskip}

Next, we prove that $\Gist$ can be constructed efficiently.

\begin{lemma}\label{lem:sizeofundirectedkernel}
    For every $i \in I'_s$, $\Gist$ can be constructed in $\widehat{O}(|V_i| \ell) = \widehat{O}( \delta \ell)$ time.
\end{lemma}
\begin{proof}
We can find $V'_i=V_i\backslash N_G[t]$ in time $\tilde O(|V_i|)$ by checking whether each node in $V_i$ is in $N_G[t]$ or not. To find $N_G[V'_i]$, for each $u\in V'_i$, list $N_G(u) \setminus N_G(s)$ and include them in $\Vist$ and also add $(u,v)$ for all $v \in N_G(u) \setminus N_G(s)$ to the set of edges, which takes time $\widehat{O}(\ell|V_i|)$ using $\cA_{recover}$ according to~\cref{cla:nearneighbor,lem:sparserecovery}. Finally, add all the edges from $t$ to $N_G(V_{s,t}^i)$.
\end{proof}


We are ready to prove \Cref{lem:datastructure}.

\begin{proof}[Proof of~\cref{lem:datastructure}]
    According to~\cref{lem:sparseneighborhoodcover}, each $v\in V$ is contained in at most $O(\log n)$ many $V_i$ for different $i$. The algorithm also returns a data structure $\cD$, according to~\cref{lem:constrcuttime}, it costs $\widehat{O}(m\delta)$ time to construct. According to~\cref{lem:sizeofundirectedkernel}, $\cD$ takes $ \widehat{O}(\delta\ell)$ time to construct the kernel $G^i_{s,t}$ for any $i\in I'_s$ (recall that $|I'_s|=O(\log n)$ according to~\cref{lem:sparseneighborhoodcover}) and we run vertex-capacity max flow calls on $G^i_{s,t}$. According to~\cref{lem:atleastkappaG}, the returned value of $\cD$ on each query $s,t$ is at least $\kappa(G)$.

    Now suppose $(L,S,R)$ is a minimum vertex cut of $G$ where $|L|\le |R|$ and $\ell\in[|L|,2|L|]$. Notice that if $|L|=\Omega(|S|)$, then the first event happens by taking $V_i=V$. Thus, in what follows we assume $|L|=o(|S|)$. We need the following claim.

    \begin{claim}
        For any $u,v\in L$, $|N_G(u)\triangle N_G(v)|\le 2|L|$.
    \end{claim}
    \begin{proof}
        We have $|N(u)\triangle N(v)|=|N(u)\cup N(v)|-|N(u)\cap N(v)|$, where $|N(u)\cup N(v)|\le |L|+|S|$, and $|N(u)\cap N(v)|=|N(u)|+|N(v)|-|N(u)\cup N(v)|$. Here $|N(u)|\ge |S|$ since $|S|$ is a minimum separator, same for $|N(v)|$. Thus, $|N(u)\cap N(v)|\ge 2|S|-(|L|+|S|)$. We have $|N(u)\triangle N(v)|\le (|L|+|S|)-(2|S|-(|L|+|S|))=2|L|$.
    \end{proof}

    We can assume WLOG that $G[L]$ is connected; otherwise, by taking a connected component of $G[L]$ we get another minimum vertex cut such that $G[L]$ is connected. According to~\cref{lem:sparseneighborhoodcover} property (cover), $L\subseteq V_i$ for some $i\in[z]$.


      We claim that if $|V_i|=\Visize$, then the second event happens. Suppose $\cD$ is given $s\in L,t\in R$, we have $|N_G(s)|=O(|L|+|S|)=O(\delta)$ since $|L|=o(|S|)$ and $|S|\le \delta$. Besides, we have $i\in I_s$ and $|V_i|\le \Visize$. Thus, according to the query algorithm for $\cD$, $\Gist$ is constructed. According to~\cref{lem:whensinLtinR}, $\cD$ will return exactly $|S|=\kappa(G)$.

        Now assume $|V_i|=\omega(\delta\log n)$, we will prove that the first event happens, i.e., $|L|=\tOm{|V_i\cap S|},|V_i\cap R|=\tOm{|V_i\cap S|}$ (remember that $L\subseteq V_i$ is already proved). If $|V_i\cap S|=O(\ell\log n)=O(|L|\log n)$, then we are done since $|V_i\cap R|=|V_i|-|L|-|V_i\cap S|=\Omega(\delta\log n)$ (remember that $\ell=\Theta(|L|)=o(|S|)=o(\delta)$).


        Now we will prove that $|V_i\cap S|=\omega(|L|\log n)$ cannot happen. We use double counting on the size of $E_G(V_i\cap S,V_i\cap R)$. we have
        \[|E_G(V_i\cap S,V_i\cap R)|\le |V_i\cap S|\cdot O(\ell\log n)\]
        since $|N_G(u)\triangle N_G(v)|=O(\ell\log n)$ according to~\cref{cla:nearneighbor} for any $u\in V_i\cap S$ (and notice that any node in $V_i\cap R$ is not a neighbor of an arbitrary vertex $v\in L$). On the other hand, consider a node $s\in L$, since $|N_G(s)|\ge |S|$ and $N_G(s)\subseteq L\cup S$, we have $|S\backslash N_G(s)|\le |L|$. Thus, we have $|V_i\cap N_G(s)|=\Theta(|V_i\cap S|)$. Now we get
        \[|E_G(V_i\cap S,V_i\cap R)|\ge \Omega(|V_i\cap R|\cdot|V_i\cap S|)\]

        since $|N_G(u)\triangle N_G(s)|=O(\ell\log n)$ for any $u\in V_i\cap R$ and $|V_i\cap N_G(s)|=\Theta(|V_i\cap S|)=\omega(\ell\log n)$. By combining the inequalities above, we get $|V_i\cap R|=O(\ell\log n)$. Thus, we have $|V_i\cap S|=|V_i|-|V_i\cap L|-|V_i\cap R|=\omega(\delta\log n)$. This is a contradiction since $|S|\le \delta$.
\end{proof}


